The Data-Production Dispositif

Machine learning (ML) depends on data to train and verify models. Very often, organizations outsource processes related to data work (i.e., generating and annotating data and evaluating outputs) through business process outsourcing (BPO) companies and crowdsourcing platforms. This paper investigates outsourced ML data work in Latin America by studying three platforms in Venezuela and a BPO in Argentina. We lean on the Foucauldian notion of dispositif to define the data-production dispositif as an ensemble of discourses, actions, and objects strategically disposed to (re)produce power/knowledge relations in data and labor. Our dispositif analysis comprises the examination of 210 data work instruction documents, 55 interviews with data workers, managers, and requesters, and participant observation. Our findings show that discourses encoded in instructions reproduce and normalize the worldviews of requesters. Precarious working conditions and economic dependency alienate workers, making them obedient to instructions. Furthermore, discourses and social contexts materialize in artifacts, such as interfaces and performance metrics, limiting workers' agency and normalizing specific ways of interpreting data. We conclude by stressing the importance of counteracting the data-production dispositif by fighting alienation and precarization, and empowering data workers to become assets in the quest for high-quality data.

==> files/reserve.tex <==
\section{Abstract}

Data production is a stepstone of machine learning that is partially outsourced through business process outsourcing companies (BPOs) and crowdsourcing platforms, a process that we call data work. Previous work has explored data work as a sense-making practice in which meaning is ascribed on datasets. This paper studies data production as a dispositif that accounts for the discourse, non-discursive practices, and materializations surrounding data work. We focused on three platforms in Venezuela and a BPO company in Argentina and analyzed annotation instructions, interviews with workers, managers, and requesters, and participant observation. Our findings show that the discursive elements in instructions, precarious working conditions, and managerial strategies ensure the perpetuation and normalization of specific discourses. We conclude by stressing the importance of democratizing data production to make worldviews encoded in datasets explicit, consider data workers as assets for high-quality data, and the necessity of empowering workers to develop ethical algorithms.

\section{related work: foucault}
%Deeply related is the concept of \emph{truth} which is described by Foucault as a system of procedures and relations that produce, regulate, and circulate discourses. A sort of feedback loop connects truth and power: while systems of power produce, sustain, and circulate truth through institutionalized discourses, the production of truth is also one technology of power which allows the institutionalization of a given discourse \cite{foucault1980}. 
%"Truth is a thing of this world: it is produced only by virtue of multiple forms of constraint. And it induces regular effects of power. (...) In societies like ours, the 'political economy' of truth is characterised by five important traits. 'Truth' is centred on the form of scientific discourse and the institutions which produce it; it is subject to constant economic and political incitement (the demand for truth, as much for economic production as for political power); it is the object, under diverse forms, of immense diffusion and consumption (circulating through apparatuses of education and information whose extent is relatively broad in the social body, not withstanding certain strict limitations); it is produced and transmitted under the control, dominant if not exclusive, of a few great political and economic apparatuses (university, army, writing, media); lastly, it is the issue of a whole political debate and social confrontation ('ideological' struggles)" \cite{foucault1980}:131-132


%Power-knowledge works as follows: Guided by their subjectivities, workers might have alternative ways of seeing and interpreting data. However, among a field of possibilities of different ways to classify, interpret and annotate data, they are guided and structured to be more likely to take particular interpretations that are preferred by the requesters.  In this sense, previous work that focuses on annotators’ subjectivity only sees this “field of possible actions” but does not see the effects of power relations, that is, annotators tend to take service requesters’ classification and interpretation of data as their only choice. Instructions shape workers because they nudge them to do as instructed. On the other hand they guide the possibilities of classification, interpretation and annotation of data and put in order the desired outcomes which is the perpetuation of pre-defined forms of truth. 
%This paper explores the mechanisms of how this takes place, that is, the dispositif. 



%Not top-down power, but disciplinary power: Admittedly, workers have their agency, though much limited, in data work, and there is a field of possible actions they can take. However, they are disciplined through institutions and strategies to take the classifications and interpretations preferred by the clients, perform annotation tasks in the way that meet the expectation and needs of service requesters, and comply with how the crowdsourcing platforms work at risk of being banned if they don't do so.

%“What I'm trying to pick out with this term is, firstly, a thoroughly heterogeneous ensemble consisting of discourses, institutions, architectural forms, regulatory decisions, laws, administrative measures, scientific statements, philosophical, moral and philanthropic propositions - in short, the said as much as the unsaid. Such are the elements of the apparatus [here dispositif is here translated as apparatus]. The apparatus itself is the system of relations that can be established between these elements. Secondly, what I am trying to identify in this apparatus is precisely the nature of the connection that can exist between these heterogeneous elements. [...] Thirdly, I understand by the term 'apparatus' a sort of -shall we say- formation which has as its major function at a given historical moment that of responding to an urgent need. The apparatus thus has a dominant strategic function.”\cite{foucault1980}:194-195

\section{Data Work}

%From the side of requesters, previous research has investigated the “large amount of work [that] goes into making data speak for themselves” \cite{passi2017}. Passi and Jackson argue that the work of data scientists combines formal knowledge and pre-established steps of analysis with situated decisions in the face of empirical contingency \cite{passi2017}.  Moreover, collaboration and negotiation among diverse actors, though often invisible, are integral to the technical operation of data science \cite{passi2018}. According to Muller et al. \cite{muller2019}, the degree of human intervention involved will determine how deep and fundamental subjective interpretations are inscribed in data. The authors argue that data scientists hardly ever receive well-structured, complete datasets and almost always need to perform complex and sometimes inventive work to make those data "whole enough" to support formal analysis. 

 %For example, in computer vision, one task for data workers involves semantic segmentation, which consists of marking and separating the different objects contained in an image \cite{Tubaro2020}. 

%Data work is circumscribed within the broader human labor necessary to develop and dispose of the material and digital infrastructures, devices, datasets, and algorithms essential for artificial intelligence. The plurality of ways humans intervene in AI was the centerpiece of the \textit{Anatomy of an AI System} by Kate Crawford and Vladan Joler \cite{Crawford2018}. In this work, Crawford and Joler map the AI labor necessary for the Amazon Alexa system to function, the natural resources involved in the production and disposal of hardware, and the data and internet infrastructures required by the system’s algorithm. The example of the Amazon Alexa shows that AI labor is plural and geographically distributed, including the humans involved in the creation of devices, from mining minerals to assembling the hardware, and from the development of algorithms by engineers and computer scientists to their training by regular users and data workers. According to Crawford and Joler \cite{Crawford2018}, this multiplicity of forms of work is also deeply tied to the environmental and natural resources required by AI, making labor and ecology deeply intertwined. 

%Several crowdsourcing startups emerged in the past decade, specializing exclusively in machine learning data work and appealing to the growing artificial intelligence market. Like other gig economy platforms, workers create an account, work as independent contractors, and are paid per task through online payment systems such as PayPal or Uphold. Instead of a manager, the work in these platforms is mediated and supervised through algorithms written by platforms’ developers \cite{Wood2018c}. In sum, this type of work presents low entry barriers and, while the piece wage is low, it is attractive in countries where the US dollar is a currency more robust than the local one. Furthermore, it allows workers to circumvent some of the geographical restrictions of local labor markets by enabling them to access work opportunities elsewhere \cite{Wood2019}.

\section{method}
\subsection{dispositif analysis}

%As described in the previous section, dispositives are systems of relations between utterances, structures, actors, and practices, in which discourses emerge and circulate. 

%Task instructions provided by requesters to data workers play a crucial role in ML data production. They prescribe specific ways of interpreting data and the realities synthesized in that data. While task instructions significantly constrain the room for worker bias, they also constitute a fundamental tool to assure the encoding of machine learning companies’ values and interests on datasets. Through they labor, data workers embed arbitrary preconceptions in training datasets by following said instructions. 

%A dispositif analysis integrates an analysis of language use with an analysis of contextual elements \cite{hamann2019}. 
%It examines how reality is brought into existence as humans assign meanings \cite{jager2016analysing}. Through this lens, material reality is not an objective given, but is constituted through ensembles of discursive and non-discursive practices as well as artifacts. 

%Through dispositif analysis, we interrogate naturalized discourses encoded in datasets.  The investigation of taken-for-granted assumptions is fundamental because “Discourse [is] an interrelated set of texts, and the practices of their production, dissemination, and reception, that brings an object into being […] In other words, social reality is produced and made real through discourses, and social interactions cannot be fully understood without reference to the discourses that give them meaning.” \cite{phillips_discourse_2002} In this sense, naturalized discourses become reality in terms of what exists within a dataset. 

%To analyze the Data Production dispositif, that is, the set of relations that determine what forms of explicit and implicit knowledge are (re)produced in the tasks data workers perform and what sort of realities machine learning datasets represent,

%For the social meaning of texts to be understood, they need to be put in relation to the wider social context in which they are used.  The combination of linguistically informed discourse analysis and sociologically informed context study was very helpful because texts and social and institutional structures refer to and constitute each other.  


%We apply the method of dispositif analysis to explore how data for machine learning is produced through outsourced labor. %the task instructions data workers follow and the interactions those instructions inform.



\section{findings}

In this subsection, we will use the framework proposed by Tubaro et al. \cite{Tubaro2020} to distinguish the different tasks available in data work. While this framework was initially conceived by analyzing digital platform labor, we consider it can also be applied to BPOs in the broader framework of data work due to the similar types of tasks available. Tubaro et al. define three moments in outsourced AI production: “artificial intelligence preparation,” “artificial intelligence verification,” and “artificial intelligence impersonation.” In the first, the authors divide AI preparation between the generation of data and its annotation. The second one involves the evaluation of algorithmic outputs. The final one, often seen in the corporate and AI-as-a-service sector \cite{Newlands2021}, refers to the non-disclosed “‘human-in-the-loop’ principle that makes workers hardly distinguishable from algorithms” \cite[7]{Tubaro2020}. This framework will complement our use of dispositif analysis to study the instructions and social relations involved in outsourced data work.

Each platforms and the BPO specialize in specific tasks that workers are instructed to perform (see Table 2). 

The language used in the instructions also depended both on the project and requester but also the platform. Workerhub, the platform with easier access for workers, requiring an email and verified PayPal account to log in, provided shorter instruction documents, consisting of a few pages, and using informal language. For example, the titles of the tasks used emoji, slang, or puns, like a task that ask workers to identify the presence of physical fights in videos titled “(ง•’\_•‘)ง Hit Me As Hard as You Can” and another task that asked workers to classify people according to perceived age titled “Is The Age Staged?” Workerhub’s instructions are short and precise, only including a brief description of the task, a definition of the taxonomy in a few lines, and many examples and counter examples. 

This approach contrasts with Tasksource, specialized in self-driving cars, whose instructions are longer, detailed, and without informal language. Instead of being presented in a few cards like in Workerhub, Tasksource workers receive handbooks as long as sixty pages and guidelines with specific details about the classifications, examples, and counter-examples. Projects in this platforms are coded with names of animals such as “Falcon” and “Zebra.” 

Despite the length and level of detail for the labels, these instructions provide little to no information about the purpose of the task. The only platform that provides this information is Clickrating. The major technology companies that outsource tasks through this platform provide long documentation like Tasksource, but also provide information about the outcome of the tasks, the company that designed it, and even the names of the employees in charge of the project. These are the only tasks that use the first person to describe the assignment. For example, one task says: “We are trying to understand the prevalence of clickbaity content News Feed. We know from research that people do not like to see clickbait in their News Feeds. If we can understand the prevalence and nature of such posts, we can better understand the News Feed ecosystem and work to improve the News Feed experience for everyone.” By contrast, Tasksource and Workerhub sometimes describe the tasks briefly and never explain their purpose.

\subsection{social practices}
\subsubsection{Obedience to Instructions}


Ronald
Por eso es que esa plataforma no me gusta tanto, porque ellos te dan las indicaciones y por más que tú sigas las indicaciones al pie de la letra, hay proyectos en donde si de verdad no lo haces perfecto, como ellos quieren o como ellos creen que es, simplemente te expulsan.

Carolina 
Entrevistador: Por ejemplo, las que son difíciles, ¿por qué es que son difíciles?
Oskarina: Porque las intenté y me botaron. Por eso es que le digo, pensé que la estaba haciendo bien y no.
Entrevistador: ¿Qué tipo de tareas eran estas?
Oskarina: Por ejemplo, ahorita hay una actividad que se llama identify runner, que selecciona los cartelitos que tenían los corredores, los que se ponen los corredores con sus números, su identificativo. Hay que seleccionarlos de la manera que ellos quieren, pero pensé que era como anteriormente lo hacía, pero no, me botaron.



Alejandro
Alejandro: Sí, había una tarea que yo creo que era para inmobiliarias, en las que había que clasificar fotos de casas dentro, fuera, seleccionar qué lugar de la casa era cada una, ahí tuve muchos problemas, pero era relativamente fácil de hacer cuando las fotos eran claras, era rápida y pagaban bien si uno hacía muchas tareas rápido.
Al mismo tiempo me gustaba, pero habían momentos en los que las fotos eran muy ambiguas, uno terminaba cometiendo errores y me expulsaron de esa tarea.
Entrevistador: ¿Tienes ejemplos de cómo eran ambiguas?
Alejandro: Sí, como dije anteriormente, ves una fachada, pero, tienes que decir-
Entrevistador: Que no sabes si está adentro o afuera.
Alejandro: -si es el patio o el exterior, o también habitaciones adentro de la casa, no se sabe si es una habitación o si es otra cosa.
Entrevistador: Esas casas, eran más que todo casas que vos dirías-- ¿Dónde crees que esas casas están?
Alejandro: En Estados Unidos, no sé en qué estado.
Entrevistador: ¿El país era Estados Unidos?
Alejandro: Sí, en Estados Unidos.

Ronald

Si yo veo que me dan, por ejemplo, este cargador y no tengo la etiqueta del adaptador, yo etiqueto solo el cargador y no etiqueto el adaptador porque no tengo una etiqueta para eso. Hay proyectos que te salen etiquetas vacío o desconocido y tú simplemente, ese objeto que no tiene etiqueta, lo etiquetas con eso.



%In our investigation, we observed all types of tasks described by Tubaro et al. \cite{Tubaro2020}, i.e., data generation, data annotation, algorithmic verification, and AI impersonation.  In the following, we describe examples of typical tasks performed by data workers at our four fieldwork sites.  The descriptions include details about how tasks are instructed to workers and how workers complete them.








%Otherness
% So, it's not new that we can't classify everything, but also thinking what is left out is important. If we keep the observation, we can see that there is an “ambiguous” or “other” category in many instructions but that there's also the non-included other. 

%Voice. CODES: Description_First-Person
%Here is the voice and the language used in classifications. Big Tech are in first person, describe the reasons why the classifications are made, while the other more exploitative platforms use the third-person and address only the task at hand. 


%Tech Jargon. CODE Description_Tech-Jargon
%También se usa mucho tech jargon que se puede dificultar a los trabajadores

%The language used in the instructions also depended both on the project and requester but also the platform. Workerhub, the platform with easier access for workers, requiring an email and verified PayPal account to log in, provided shorter instruction documents, consisting of a few pages, and using informal language. For example, the titles of the tasks used emoji, slang, or puns, like a task that ask workers to identify the presence of physical fights in videos titled “(ง•’\_•‘)ง Hit Me As Hard as You Can” and another task that asked workers to classify people according to perceived age titled “Is The Age Staged?” Workerhub’s instructions are short and precise, only including a brief description of the task, a definition of the taxonomy in a few lines, and many examples and counter examples. This approach contrasts with Tasksource, specialized in self-driving cars, whose instructions are longer, detailed, and without informal language. Instead of being presented in a few cards like in Workerhub, Tasksource workers receive handbooks as long as sixty pages and guidelines with specific details about the classifications, examples, and counter-examples. Projects in this platforms are coded with names of animals such as “Falcon” and “Zebra.”  Despite the length and level of detail for the labels, these instructions provide little to no information about the purpose of the task. The only platform that provides this information is Clickrating. The major technology companies that outsource tasks through this platform provide long documentation like Tasksource, but also provide information about the outcome of the tasks, the company that designed it, and even the names of the employees in charge of the project. These are the only tasks that use the first person to describe the assignment. For example, one task says: “We are trying to understand the prevalence of clickbaity content News Feed. We know from research that people do not like to see clickbait in their News Feeds. If we can understand the prevalence and nature of such posts, we can better understand the News Feed ecosystem and work to improve the News Feed experience for everyone.” By contrast, Tasksource and Workerhub sometimes describe the tasks briefly and never explain their purpose.



%For-profit priorities CODES: Labels_Definitions, Labels_Other-Unkknown
% Here we can say that, of course, classficiations have a commercial application. Like, if you're building a self-driving car, your classifications will be aimed at objects found by cars. That said, we can argue that we did not observe static classifications but that they evolve, and they should evolve. Two examples: a classification made to moderate image content in Hive had to be trasnformed to include videos as well. 
%US-centric worldviews. CODES: Labels_Definitions but also in the INTERVIEWS/Tasks_Classification-Categorization
% Product classification have categories relevant to the US, which in itself is not a bad thing, but it makes the task difficult for workers

% ======================================


